Exploring Connections Between Active Learning and Model Extraction

Machine learning is being increasingly used by individuals, research institutions, and corporations. This has resulted in the surge of Machine Learning-as-a-Service (MLaaS) - cloud services that provide (a) tools and resources to learn the model, and (b) a user-friendly query interface to access the model. However, such MLaaS systems raise privacy concerns such as model extraction. In model extraction attacks, adversaries maliciously exploit the query interface to steal the model. More precisely, in a model extraction attack, a good approximation of a sensitive or proprietary model held by the server is extracted (i.e. learned) by a dishonest user who interacts with the server only via the query interface. This attack was introduced by Tramer et al. at the 2016 USENIX Security Symposium, where practical attacks for various models were shown. We believe that better understanding the efficacy of model extraction attacks is paramount to designing secure MLaaS systems. To that end, we take the first step by (a) formalizing model extraction and discussing possible defense strategies, and (b) drawing parallels between model extraction and established area of active learning. In particular, we show that recent advancements in the active learning domain can be used to implement powerful model extraction attacks, and investigate possible defense strategies.

==> Anon_Contents/Nonlinear.tex <==
\section{Non-linear Classifiers}
\label{sec:non-linear}

This section focuses on model theft for two important non-linear
classifiers: kernel SVMs and discrete models (\ie decision trees and
random forests). For kernel SVMs our method is a combination of the
adaptive-retraining algorithm introduced by Tram\`{e}r \etal and the
active selection strategy from classic literature on active
learning of kernel SVMs~\cite{LASVM}. For discrete models our
algorithm is based on the importance weighted active learning (IWAL)
as described in~\cite{iwal:2010}. Note that decision trees
for general labels (\ie non-binary case) and random forests was not
discussed in~\cite{iwal:2010}.


\subsection{Kernel SVMs}
\label{subsec:kSVM}

In kernel SVMs (kSVMs), there is a kernel $K:\X\times\X\rightarrow\R$ associated with the
SVM. Some of the common kernels are polynomials and radial-basis
functions (RBFs). If the kernel function $K(.,.)$ has some special
properties (required by classic theorem of Mercer), then $K(.,.)$ can
be written as $\Phi (.)^T \Phi(.)$ for a projection/feature function $\Phi$. In
the feature space (the domain of $\Phi$) the optimization problem is
as follows\footnote{we are using the formulation for soft-margin kSVMs}:
\[
\begin{array}{c}
  \mbox{min}_{w,b} \| w \|^2 + C \sum_{i=1}^n \eta_i \\
  \mbox{such that for $1 \leq i \leq n$} \\
  y_i \hat{y}(x_i) \; \geq \; 1 - \eta_i \\
  \eta_i \; \geq 0
\end{array}
\]
In the formulation given above, $\hat{y}(x)$ is equal to $w^T \Phi(x) +
b$. Recall that prediction of the kSVM is the sign of $\hat{y}(x)$, so
$\hat{y}(x)$ is the ``pre sign'' value of the prediction. Note that
for some kernels (\eg RBF) $\Phi$ is infinite dimensional, so one
generally uses the ``kernel trick''\ie one solves the dual of
the above problem and obtains a {\it kernel expansion}, so that
\begin{eqnarray*}
  \hat{y}(x) & = & \sum_{i=1}^n \alpha_i K(x,x_i) \; + \; b
\end{eqnarray*}
The vectors $x_1,\cdots,x_n$ are called support vectors.
We assume that hyper-parameters of
the kernel ($C, \eta$) are known ( one can extract the hyper-parameters for
the RBF kernel using the extract-and-test approach as Tram\`{e}r \etal)
Note that if $\Phi$ is finite dimensional, we can use an algorithm (including active learning strategies)
for linear classifier by simply working in the feature space (\ie
the domain of $\Phi(\cdot)$). However, there is a subtle issue here, which
was not addressed by Tram\`{e}r \etal We need to make sure that if a query
$y$ is made in the feature space, it is ``realizable'' (\ie there exists
a $x$ such that $\Phi (x) = y$). Otherwise the learning algorithm
is not sound. 

Next we describe our model-extraction algorithm for kSVMs with kernels
whose feature space is infinite dimension (\eg RBF or Laplace
kernels). Our algorithm is a modification of the adaptive training
approach from Tram\`{e}r \etal Our discussion is specialized to kSVMs with
RBFs, but our ideas are general and are applicable in other
contexts.

\noindent
%Adaptive training was introduced by Tram\`{e}r \etal~\cite{TZJRR16}. We extend their method (hence the name), and show that these extensions can improve query complexity. 
{\bf Extended Adaptive Training (EAT):} EAT proceeds in multiple rounds. In each round we
construct $h$ labeled samples. In the initial stage ($t=0$) we draw $r$
samples $x_1,\cdots,x_r$ from the uniform distribution, query their
labels, and create an initial model $M_0$. Assume that we are at round
$t$, where $t > 0$, and let $M_{t-1}$ be model at time $t-1$. Round
$t$ works as follows: create $h$ labeled samples using a strategy
$St^{\mathcal{T}} (M_{t-1},h)$ (note that the strategy $St$ is oracle
access to the teacher, and takes as parameters model from the previous
round and number of labeled samples to be generated). Now we train
$M_{t-1}$ on the samples in $St^{\mathcal{T}} (M_{t-1},h)$ and obtain
the updated model $M_t$. We keep iterating using the strategy
$St^{\mathcal{T}} (\cdot,\cdot)$ until the query budget is
satisfied. Ideally, $St^{\mathcal{T}} (M_{t-1},h)$ should be samples
that the model $M_{t-1}$ is ``least confident'' about or closest to the decision
boundary. The challenge lies in finding these uncertain points. % close to the decision boundary? This is where we differ and generalize Tram\`{e}r's method.

Tram\`{e}r \etal use line search as their strategy $St^{\mathcal{T}}
(M_{t-1},h)$, which can lead to several queries (each step in the binary
search leads to a query). We generate the initial model $M_0$ as in
Tram\`{e}r \etal and then our strategy differs.  Our strategy
$St^{\mathcal{T}}(M_{t-1},1)$ (note that we only add one labeled
sample at each iteration) works as follows: we generate $k$ random
points $x_1,\cdots,x_k$ and then compute $\hat{y_i}(x_i)$ for each
$x_i$ (recall that $\hat{y_i}(x_i)$ is the ``pre sign'' prediction of
$x_i$ on the SVM $M_{t-1}$. We then pick $x_i$ with minimum $\mid
\hat{y_i}(x_i) \mid$ and query for its label and retrain the model
$M_{t-1}$ and obtain $M_t$. This strategy is called {\it active
  selection} and has been used active learning for
SVMs~\cite{LASVM}. The argument for why this strategy finds the point
closest to the boundary is given in~\cite[Section 4]{LASVM}. There are
other strategies described in~\cite{LASVM}, but we found that active
selection performs the best.

\subsection{Decision Trees and Random Forests}
\label{subsec:iwal}


Next we will describe the idea of {\it importance weighted active
  learning (IWAL)}. Our discussion will be specialized to decision
trees and random forests, but the ideas that are described are
general~\cite{iwal:2010}.

Let $\mathcal{H}$ be the hypothesis class (\ie space of decision
trees or random forests), $\X$ is the space of data, and
$\Y$ is the space of labels.  The active learner has a pool
of unlabeled data $x_1,x_2,\cdots$. For $i > 1$, we denote by
$X_{1:i-1}$ the sequence $x_1,\cdots,x_{i-1}$. After having processed the sequence
$X_{1:i-1}$, a coin is flipped with probability $p_i \in [0,1]$ and
if it comes up heads, the label of $x_i$ is queried. We also define a set
$S_i$ ($S_0 = \emptyset$) recursively as follows: If the label for
$x_i$ is not queried, then $S_i \; = \; S_{i-1}$; otherwise $S_i \; =
\; S_{i-1} \cup {(x_i,y_i,p_i)}$. Essentially the set $S_i$ keeps the
information (\ie data, label, and probability of querying) for all
the datapoints whose label was queried. Given a hypothesis $h \in \mathcal{H}$,
we define $err(h,S_n)$ as follows:
\begin{eqnarray}
  err(h,S_n) & = & \frac{1}{n} \sum_{(x,y,p) \in S_n} \frac{1}{p} 1_{h(x) \not= y}
\end{eqnarray}
Next we define the following quantities (we assume $n \geq 1$):
\begin{eqnarray*}
  h_n & = & \mbox{argmin} \{ err(h,S_{n-1}) \; : \; h \in \mathcal{H} \} \\
  h'_n & = & \mbox{argmin} \{ err(h,S_{n-1}) \; : \; h \in \mathcal{H} \wedge h(X_n) \not= h_n (X_n) \} \\
  G_n & = & err(h'_n,S_{n-1}) - err(h_n,S_{n-1})
\end{eqnarray*}
Recall that $p_n$ is the probability of querying for the label for
$X_n$, which is defined as follows:
\[
p_n = \left\{ \begin{array}{ll}
  1 & \mbox{if $G_n \leq \mu(n)$} \\
  s(n) & \mbox{otherwise}
  \end{array}
  \right.
  \]
  Where $\mu (n) = \sqrt{ \frac{c_0 \log n}{n-1} } + \frac{c_0 \log n}{n-1}$, and $s(n) \in (0,1)$
  is the positive solution to the following equation:
  \begin{eqnarray*}
    G_n & = & \left( \frac{c_1}{\sqrt{s} - c_1 + 1} \right) \cdot   \sqrt{ \frac{c_0 \log n}{n-1} }  +
    \left( \frac{c_2}{\sqrt{s} - c_2 + 1} \right) \cdot  \frac{c_0 \log n}{n-1}
  \end{eqnarray*}
  Note the dependence on constants/hyperparameters $c_0$, $c_1$ and
  $c_2$, which are tuned for a specific problem (\eg in their
  experiments for decision trees~\cite[Section 6]{iwal:2010} the
  authors set $c_0=8$ and $c_1 = c_2 = 1$).


  \noindent
      {\bf Decision Trees:} Let $DT$ be any algorithm to create a
      decision tree. We start with an initial tree $h_0$ (this can
      constructed using a small, uniformly sampled dataset whose labels are queried). Let
      $h_n$ be the tree at step $n-1$. The question is: how to
      construct $h'_n$? Let $x_n$ be the $n$-th datapoint and $\Y
      = \{ l_1,\cdots,l_r \}$ be the set of labels. Let $h_n (x_n) =
      l_j$. Let $h_n (l)$ be the modification of tree $h_n$ such that
      $h_n (l)$ produces label $l \not= h_n (x_n)$ on datapoint $x_n$. Let
      $h'_n$ be the tree in the set $\{ h_n (l) \; | \; l \in \Y-\{
      l_j \} \}$ that has minimum $err(\cdot,S_{n-1})$. Now we can
      compute $G_n$ and the algorithm can proceed as described before.

      \noindent
          {\bf Random Forests:} In this case we will restrict
          ourselves to binary classification, but the algorithm can
          readily extended to the case of multiple labels. As before
          $RF_0$ is the random forest trained on a small initial
          dataset. Since we are in the binary classification domain, the
          label set $\Y = \{ 1,-1 \}$. Assume that we have a
          random forest $RF = \{ RF[1],\cdots,RF[o] \}$ of trees
          $RF[i]$ and on a datapoint $x$ the label of $RF(x)$ is the
          majority of the label of the trees $RF[1] (x),\cdots,
          RF[o](x)$. Let $RF_n$ be the random forest at time step
          $n-1$. The question again is: how to construct $RF'_n$?
          Without loss of generality, let us say on $x_n$ $RF_n (x_n) = +1$ (the case when
          the label is $-1$ is symmetric) and there are $r$ trees in
          $RF_n$ (denoted by $RF_n^{+1} (x_n)$) such that their labels
          on $x_n$ are $+1$. Note that $r > \lfloor \frac{o}{2}
          \rfloor $ because the majority label was $+1$. Define $j =
          r-\lfloor \frac{o}{2} \rfloor+1$.  Note that if $j$ trees in
          $RF^{+1}_n (x_n)$ will ``flip'' their decision to $-1$ on $x_n$, then
          the decision on $x_n$ will be flipped to $-1$. This is the
          intuition we use to compute $RF'_n$. %We pick $j$ trees out of $RF_n^{+1} (x_n)$ and flip their decisions to $-1$. 
          There are ${r \choose j}$ choices of trees and we pick the one
          with minimum error on $S_{n-1}$, and that gives us $RF'_n$.
          Recall that $r \choose j$ is approximately $r^j$, but we can
          be approximate by randomly picking $j$ trees out of $RF_n^{+1}
          (x_n)$, and choosing the random draw with the minimum
          error to approximate $RF'_n$.
  



==> Anon_Contents/Songbai/proof.tex <==
\section{Settings}

Assume unit vector $u\in\mathbb{R}^{d}$ is the groundtruth. For each
query $x\in\mathbb{R}^{d}$, a vector $w$ is drawn from $N(u,\sigma^{2}I)$,
and the label $y=\text{sign}(\left\langle w,x\right\rangle )$ is
returned. The goal of the learner (attacker) is to return $\hat{w}$
such that $\left\Vert u-\hat{w}\right\Vert $ is small.

\section{Algorithm}

The attacking algorithm is as shown as Algorithm~\ref{alg:passive}.
It takes an estimated upper bound $\hat{\sigma}$ of $\sigma$ as
input. The algorithm first draws $m=\tilde{O}(\frac{d}{\varepsilon^{2}}\max(1,d\hat{\sigma}^{2}))$
labeled examples $\{(x_{i},y_{i})\}_{i=1}^{m}$ from the unit sphere
uniformly at random, and then computes the average $v=\sum_{i=1}^{m}y_{i}x_{i}$.
$\ensuremath{\hat{w}=\frac{v}{\left\Vert v\right\Vert }}$, the direction
of $v$ is the algorithm's estimate of the classifier $u$, and the
length of $v$ is used as an indicator of whether the algorithm succeeds:
if this estimated upper bound is correct (i.e. $\sigma\leq\hat{\sigma}$),
then with high probability, $\left\Vert \hat{w}-u\right\Vert \leq\varepsilon$;
otherwise it outputs \textsc{fail}, indicating the variance bound $\hat{\sigma}$
is incorrect.

\begin{algorithm}
\begin{algorithmic}[1]
\State{Input: variance upper bound $\hat{\sigma}\geq \frac{1}{\sqrt{d}}$, target error $\varepsilon$}
\State{$m \gets \frac{(15\pi)^2}{\varepsilon^2}d\max(1,d\hat{\sigma}^2)\log\frac{2d}{\delta}$, $l \gets \frac{1}{12d\hat{\sigma}}$}
\State{Draw $x_1,x_2,\dots,x_m\in\mathbb{S}^{d-1}$ uniformly at random, and query their labels $y_1,y_2,\dots,y_m$}
\State{$v \gets \sum_{i=1}^m y_i x_i$}
\If{$\left\Vert v\right\Vert \geq l$}
\State{Return $\hat{w}=\frac{v}{\left\Vert v\right\Vert}$}
\Else
\State{Return \textsc{fail}}
\EndIf
\end{algorithmic}

\caption{\label{alg:passive}Attacking Algorithm}
\end{algorithm}

\section{Analysis}

We have following theoretical guarantees for Algorithm~\ref{alg:passive}.
\begin{proposition}
\label{proposition:complexity}If $\sigma\leq\hat{\sigma}$, then $\left\Vert \hat{w}-u\right\Vert \leq\varepsilon$
with probability at least $1-\delta$.
\end{proposition}

\begin{proposition}
\label{proposition:length-lb}If $\sigma\leq\hat{\sigma}$ and $\hat{\sigma}\geq\frac{1}{\sqrt{d}}$,
then $\left\Vert v\right\Vert \geq\frac{1}{12d\hat{\sigma}}$ with
probability at least $1-\delta$.
\end{proposition}

\begin{proposition}
\label{proposition:length-ub}If $\sigma\geq20\hat{\sigma}\geq\frac{1}{\sqrt{d}}$,
then $\left\Vert v\right\Vert \leq\frac{1}{\sqrt{148}d\hat{\sigma}}$
with probability at least $1-\delta$.
\end{proposition}

propositionositions~\ref{proposition:complexity} and \ref{proposition:length-lb} guarantees
that if the estimated upper bound is correct ($\sigma\leq\hat{\sigma}$),
then the algorithm outputs an accurate estimation of $u$; propositionosition~\ref{proposition:length-ub}
guarantees the algorithm declares failure if the estimated upper bound
is too small ($\hat{\sigma}\leq\frac{1}{20}\sigma$).

Intuitively, the average of $y_{i}x_{i}$ ($i=1,\dots,m$) points
to a direction similar to $u$ because of the symmetry of distributions
of both $x$ and noise: the projection of $yx$ onto all directions
perpendicular to $u$ is distributed symmetrically around 0 and thus
has mean 0. The projection of $yx$ onto $u$ has non-negative mean
since the label $y$ is correct (i.e., $yv^{\top}x\geq0$) with probability
at least $\frac{1}{2}$, and the projection is larger if the noise
of $y$ is smaller. Consequently, the scale of the average can be
used as an indicator of the noise level. The propositionositions can be formally
proved by applying concentration inequalities on each direction.

\section{Proofs}

Denote by $\mathbb{S}^{d-1}$ the unit sphere $\{x\in\R^{d}:x^{\top}x=1\}$.
For any vector $X\in\R^{d}$, denote by $X^{(i)}$ the $i$-th coordinate
of $X$. Define $Z_{i}=Y_{i}X_{i}$ for $i=1,2,\dots,m$.

We need following facts.
\begin{fact}
\label{fact:gaussian}$\Pr(w^{\top}x\geq0)=\Pr_{\xi\sim N(0,1)}(\xi\geq-\frac{w^{\star\top}x}{\sigma\left\Vert x\right\Vert })$.
Moreover, for $z\geq0$, $\frac{1}{2}-\frac{z}{\sqrt{2\pi}\sigma}\leq\Pr_{\xi\sim N(0,1)}(\xi\geq\frac{z}{\sigma})\leq\max(\frac{1}{6},\frac{1}{2}-\frac{z}{3\sigma})$.
\end{fact}

\begin{fact}
\label{fact:beta}Let $B(x,y)=\int_{0}^{1}(1-t)^{x-1}t^{y-1}dt$ be
the Beta function. Then $\frac{2}{\sqrt{d-1}}\leq B(\frac{1}{2},\frac{d}{2})\leq\frac{\pi}{\sqrt{d}}$.
\end{fact}

\begin{fact}
\label{fact:exp}If $d\geq2$, then $(1-\frac{1}{d})^{\frac{d}{2}}\geq\frac{1}{2}$.
\end{fact}

\begin{fact}
(Bernstein inequality) If i.i.d. random variables $X_{1},\dots,X_{m}$
satisfy $|X_{i}|\leq b$, $\E[X_{i}]=\mu$, and $\E[X_{i}^{2}]\leq r^{2}$,
then with probability at least $1-\delta$, $|\frac{1}{m}\sum_{i=1}^{m}X_{i}-\mu|\leq\sqrt{\frac{2r^{2}}{m}\log\frac{2}{\delta}}+\frac{2b}{3m}\log\frac{2}{\delta}$.
\end{fact}

\begin{fact}
\label{fact:density}Suppose $(x_{1},\dots,x_{d})$ is drawn from
the uniform distribution over the unit sphere, then $x_{1}$ has a
density function of $p(z)=\frac{(1-z^{2})^{\frac{d-3}{2}}}{B(\frac{d-1}{2},\frac{1}{2})}$.
\end{fact}

Without loss of generality, assume $u=(1,0,0,\dots,0)$. 

Following three lemmas give concentration of $v$.
\begin{lemma}
\label{lem:ub-k}For any $k=2,3,\dots,d$, with probability at least
$1-\delta$, $|v^{(k)}|\leq2\sqrt{\frac{2}{md}\log\frac{2}{\delta}}$.
\end{lemma}

\begin{proof}
For $k=2,3,\dots,d$, $Z_{1}^{(k)},Z_{2}^{(k)},\dots,Z_{m}^{(k)}$
are i.i.d. random variables bounded by 1. By symmetry, $\E[Z_{1}^{(k)}]=0$.
$\E[(Z_{1}^{(k)})^{2}]=\E[(X^{(i)})^{2}]=2\int_{0}^{1}z^{2}\frac{(1-z^{2})^{\frac{d-3}{2}}}{B(\frac{d-1}{2},\frac{1}{2})}dz=\frac{1}{B(\frac{d-1}{2},\frac{1}{2})}\int_{0}^{1}t^{\frac{1}{2}}(1-t)^{\frac{d-3}{2}}dt=\frac{B(\frac{d-1}{2},\frac{3}{2})}{B(\frac{d-1}{2},\frac{1}{2})}=\frac{1}{d}$.
By the Bernstein inequality, with probability at least $1-\delta$,
$|\frac{1}{m}\sum Z_{i}^{(k)}|\leq\sqrt{\frac{2}{md}\log\frac{2}{\delta}}+\frac{2}{3m}\log\frac{2}{\delta}\leq2\sqrt{\frac{2}{md}\log\frac{2}{\delta}}$.
\end{proof}
\begin{lemma}
\label{lem:lb-1}With probability at least $1-\delta$, $v^{(1)}\geq\frac{1}{3\pi\sqrt{d}}\min(1,\frac{1}{\sigma\sqrt{d}})-\sqrt{\frac{1}{2m}\log\frac{1}{\delta}}$.
\end{lemma}

\begin{proof}
$Z_{1}^{(1)},Z_{2}^{(1)},\dots,Z_{m}^{(1)}$ are i.i.d. random variables
bounded by 1. Their mean can be lower-bounded as follows. 

For for any $0\leq a\leq1$, due to the noise setting, $\E[Y\mid X^{(1)}=a]\geq0$
and $\E[Y\mid X^{(1)}=-a]\leq0$, so $\E[YX^{(1)}\mid X^{(1)}=a]+\E[YX^{(1)}\mid X^{(1)}=-a]\geq0$.
Consequently we have

\begin{align*}
\text{TEXT COMMENTED HERE IN ORDER TO COMPILE!}
%\E[YX^{(1)}] & \geq\E[YX^{(1)}\One[|X^{(1)}|\geq\frac{1}{\sqrt{d}}]]\\
% & =\E[\E[Y\mid X^{(1)}]X^{(1)}\One[|X^{(1)}|\geq\frac{1}{\sqrt{d}}]]\\
%& =\E[(1-2\Pr[Y=-1\mid X^{(1)}])X^{(1)}\One[X^{(1)}\geq\frac{1}{\sqrt{d}}]]\\
% & \geq(1-2\Pr_{\xi\sim N(0,1)}(\xi\geq\frac{1}{\sigma\sqrt{d}}))\E[X^{(1)}\One[X^{(1)}\geq\frac{1}{\sqrt{d}}]]
\end{align*}

Now, $\Pr_{\xi\sim N(0,1)}(\xi\geq\frac{1}{\sigma\sqrt{d}})\leq\max(\frac{1}{6},\frac{1}{2}-\frac{1}{3\sigma\sqrt{d}})$.
Besides,  TEXT COMMENTED HERE IN ORDER TO COMPILE! %$\E[X^{(1)}\One[X^{(1)}\geq\frac{1}{\sqrt{d}}]]=\int_{\frac{1}{\sqrt{d}}}^{1}\frac{z(1-z^{2})^{\frac{d-3}{2}}}{B(\frac{d-1}{2},\frac{1}{2})}dz=\frac{(1-\frac{1}{d})^{\frac{d-1}{2}}}{(d-1)B(\frac{d-1}{2},\frac{1}{2})}\geq\frac{1}{2(d-1)\frac{\pi}{\sqrt{d-1}}}\geq\frac{1}{2\pi\sqrt{d}}$
where the first inequality follows by Fact~\ref{fact:beta} and \ref{fact:exp}.
Thus, $\E[YX^{(1)}]\geq\frac{1}{3\pi\sqrt{d}}\min(1,\frac{1}{\sigma\sqrt{d}})$. 

By the Chernoff bound, with probability at least $1-\delta$, $v^{(1)}=\frac{1}{m}\sum Z_{i}^{(1)}\geq\frac{1}{3\pi\sqrt{d}}\min(1,\frac{1}{\sigma\sqrt{d}})-\sqrt{\frac{1}{2m}\log\frac{1}{\delta}}$.
\end{proof}
\begin{lemma}
\label{lem:ub-1}With probability at least $1-\delta$, $v^{(1)}\leq\frac{2}{\sqrt{2\pi}d\sigma}+\sqrt{\frac{1}{2m}\log\frac{1}{\delta}}$.
\end{lemma}

\begin{proof}
We first give an upper bound of $\E[YX^{(1)}]=2\int_{0}^{1}z\frac{(1-z^{2})^{\frac{d-3}{2}}}{B(\frac{d-1}{2},\frac{1}{2})}(1-2\Pr_{\xi\sim N(0,1)}(\xi\geq\frac{z}{\sigma}))dz$.
By Fact~\ref{fact:gaussian}, $1-2\Pr_{\xi\sim N(0,1)}(\xi\geq\frac{z}{\sigma})\leq\frac{2z}{\sqrt{2\pi}\sigma}$,
so we have

\begin{align*}
\E[YX^{(1)}] & \leq2\int_{0}^{1}z\frac{(1-z^{2})^{\frac{d-3}{2}}}{B(\frac{d-1}{2},\frac{1}{2})}\frac{2z}{\sqrt{2\pi}\sigma}dz\\
 & =\frac{4}{\sqrt{2\pi}\sigma B(\frac{d-1}{2},\frac{1}{2})}\int_{0}^{1}z^{2}(1-z^{2})^{\frac{d-3}{2}}dz\\
 & =\frac{2B(\frac{d-1}{2},\frac{3}{2})}{\sqrt{2\pi}\sigma B(\frac{d-1}{2},\frac{1}{2})}\\
 & =\frac{2}{\sqrt{2\pi}d\sigma}
\end{align*}

The conclusion follows by the Chernoff bound.
\end{proof}
Now we present the proofs for the propositionositions.
\begin{proof}
(of propositionosition~\ref{proposition:complexity}) Since $\left\Vert \hat{w}-u\right\Vert ^{2}=\left\Vert \hat{w}\right\Vert ^{2}+\left\Vert u\right\Vert ^{2}-2u^{\top}\hat{w}=2(1-u^{\top}\hat{w})=2(1-\frac{v^{(1)}}{\left\Vert v\right\Vert })$,
to prove $\left\Vert \hat{w}-u\right\Vert \leq\varepsilon$, it suffices
to show $\frac{v^{(1)}}{\left\Vert v\right\Vert }\geq1-\frac{\varepsilon^{2}}{2}$.
Note that $1-(\frac{v^{(1)}}{\left\Vert v\right\Vert })^{2}=\frac{1}{1+\frac{(v^{(1)})^{2}}{\sum_{k=2}^{d}(v^{(k)})^{2}}}$,
and $1-(1-\frac{\varepsilon^{2}}{2})^{2}=\varepsilon^{2}-\frac{\varepsilon^{4}}{4}\geq\frac{\varepsilon^{2}}{2}\geq\frac{1}{1+\frac{2}{\varepsilon^{2}}}$
, so it suffices to show $\frac{(v^{(1)})^{2}}{\sum_{k=2}^{d}(v^{(k)})^{2}}\geq\frac{2}{\varepsilon^{2}}$
with probability at least $1-\delta$.

Now, by Lemma~\ref{lem:ub-k} and \ref{lem:lb-1} and a union bound,
with probability at least $1-\delta$,
\[
\frac{(v^{(1)})^{2}}{\sum_{k=2}^{d}(v^{(k)})^{2}}\geq\frac{(\frac{1}{3\pi\sqrt{d}}\min(1,\frac{1}{\sigma\sqrt{d}})-\sqrt{\frac{1}{2m}\log\frac{d}{\delta}})^{2}}{4(d-1)\frac{2}{md}\log\frac{2d}{\delta}},
\]

which is at least $\frac{2}{\varepsilon^{2}}$ for our setting of $m=\frac{(15\pi)^{2}}{\varepsilon^{2}}d\max(1,d\hat{\sigma}^{2})\log\frac{2d}{\delta}$.
\end{proof}
%
\begin{proof}
(of propositionosition~\ref{proposition:length-lb}) By Lemma~\ref{lem:lb-1},
with probability at least $1-\delta$, $v^{(1)}=\frac{1}{m}\sum Z_{i}^{(1)}\geq\frac{1}{3\pi\sqrt{d}}\min(1,\frac{1}{\sigma\sqrt{d}})-\sqrt{\frac{1}{2m}\log\frac{1}{\delta}}\geq\frac{1}{12\sqrt{d}}\min(1,\frac{1}{\hat{\sigma}\sqrt{d}})$,
which implies $\left\Vert v\right\Vert \geq v^{(1)}\geq\frac{1}{12\sqrt{d}}\min(1,\frac{1}{\hat{\sigma}\sqrt{d}})$.
\end{proof}
%
\begin{proof}
(of propositionosition~\ref{proposition:length-ub}) By Lemma~\ref{lem:ub-k}
and \ref{lem:ub-1} and a union bound, with probability at least $1-\delta$,

\begin{align*}
\left\Vert v\right\Vert ^{2} & =\sum_{k=1}^{d}(v^{(k)})^{2}\\
 & \leq4(d-1)\frac{2}{md}\log\frac{2d}{\delta}+(\frac{2}{\sqrt{2\pi}d\sigma}+\sqrt{\frac{1}{2m}\log\frac{1}{\delta}})^{2}\\
 & \leq\frac{1}{148d^{2}\hat{\sigma}^{2}}.
\end{align*}
\end{proof}


==> Anon_Contents/Songbai/theory.tex <==
\section{Model Extraction with a General Model Class}

From a learning theoretical perspective, we can formulate the general
model extraction problem as follows: Suppose there is an underlying
data distribution $D$ over $\mathcal{X}\times\mathcal{Y}$, a hypothesis
class $\mathcal{H}$ of VC dimension $d$\footnote{The VC dimension of a hypothesis
class $\mathcal{H}$ is the largest number $d$ such that there exists a subset $X\subset\mathcal{X}$ of size $d$ which can be shattered by $\mathcal{H}$. An example set $X=\{x_1, \dots, x_d\}\subset\mathcal{X}$ is said to be shattered by $\mathcal{H}$ if $|\{(h(x_1), h(x_2),\dots,h(x_d)):h\in\mathcal{H}\}|=2^d$.}, and a ground-truth classifier
$h^{\star}\in\mathcal{H}$. The goal of the learner is to find a classifier $h$
such that $\Pr_{(X,Y)\sim D}(h(X)\neq Y)\leq\Pr_{(X,Y)\sim D}(h^{\star}(X)\neq Y)+\varepsilon$.

\begin{remark}
$\Pr_{D}(X)$ can be assumed to be uniform over some space since we
have no training data distribution in model extraction. The defender has $h^{*}$ and wishes to protect it. To protect $h^{*}$, for each query $x\in\mathcal{H}$, instead of returning $h^{*}(x)$, the defender returns a label $y$ drawn from the distribution $\Pr_{D}(Y\mid X=x)$. $\Pr_{D}(Y\mid X)$, which characterizes the query-answering strategy of the defender, can be any distribution. $\Pr(h^{\star}(X)\neq Y)$ indicates the noise level added by the defender. The attacker wishes to find an $h$ that is close to $h^\star$. The performance of $h$ is measured by $\Pr_D(h(X)\neq Y)$, the capability of predicting $Y$ given $X$. Since the defender adds noise to labels, the attacker only needs to achieve a low error rate ralative to $h^\star$, that is, $\Pr_{(X,Y)\sim D}(h^{\star}(X)\neq Y)+\varepsilon$.

In the passive learning setting, the learner (attacker) draws
examples from $D$ to query for labels. In the membership active learning setting, the learner can interactively query any examples $x$ from the sample space $\mathcal{X}$.
\end{remark}

\begin{definition}
In this note, all probabilities are over $D$, and we drop subscript
$D$ from $\Pr_{D}$ henceforth. Define $l(h):=\Pr(h(X)\neq Y)$,
$\nu:=\Pr(h^{\star}(X)\neq Y)$. 
\end{definition}
We next present some known results which ignores computational cost
(i.e., algorithms that achieve the bounds do not run in polynomial
time) \cite{key-1}. These results establish information theoretical
bounds for the number of queries required to extract the model.

\paragraph{Passive Learning}

%%%% IRENE: what is the command \One in the footnote ???????/

The Empirical Risk Minimization algorithm\footnote{TEXT COMMENTED IN THE FOOTNOTE IN ORDER TO COMPILE!}
	%\footnote{Given a labeled training set $\{(X_1,Y_1),\dots(X_n,Y_n)\}$, the Empirical Risk Minimization algorithm outputs $\hat{h}=\arg\min_{h\in\mathcal{H}}\frac1n \sum_{i=1}^n \One[h(X_i)\neq Y_i]$.} 
returns $\hat{h}$ with excess error $\varepsilon$ (i.e.,
$l(\hat{h})\leq\nu+\varepsilon$) with $\tilde{O}(\frac{\nu+\varepsilon}{\varepsilon^{2}}d)$
examples. For any algorithm, there is a distribution such that the
algorithm needs at least $\tilde{\Omega}(\frac{\nu+\varepsilon}{\varepsilon^{2}}d)$
samples to achieve an excess error of $\varepsilon$.

\paragraph{Active Learning}

The disagreement-based active learning algorithm \cite{key-1} achieves excess error
$\varepsilon$ with $\tilde{O}(\frac{\nu^{2}}{\varepsilon^{2}}d\theta)$
queries (where $\theta$ is the disagreement coefficient). For any
active learning algorithm, there is a distribution such that it takes
at least $\tilde{\Omega}(\frac{\nu^{2}}{\varepsilon^{2}}d)$ queries
to achieve an excess error of $\varepsilon$.

\section{Model Extraction with Linear Models}

Now, we restrict the hypothesis class $\mathcal{H}$ to be homogeneous
(i.e., the classification hyperplane passes the origin) linear classifiers
in $\mathbb{R}^{d}$.

In general, learning linear models with agnostic noise (i.e., no assumption
on the noise) is computationally hard \cite{key-2,key-3}. Some positive
results exist under moderate noise conditions. Under random classification
noise where each label is flipped with probability exactly $\eta$,
the AVERAGE algorithm (similar to ours) needs $\tilde{O}(\frac{d^{2}}{(1-2\eta)^{2}}\log\frac{1}{\varepsilon})$
labels \cite{key-3}. Under bounded noise where each label is flipped
with probability at most $\eta$, the AVERAGE algorithm does not work
anymore, but a modified Perceptron algorithm can learn with $\tilde{O}(\frac{d}{(1-2\eta)^{2}}\log\frac{1}{\varepsilon})$
labels \cite{key-5}. Under the adversarial noise where $\nu=\Omega(\varepsilon)$,
\cite{key-6} proposes an algorithm that minimizes a sequence of hinge
losses and uses $\tilde{O}(d\log\frac{1}{\varepsilon})$ labels.
\begin{remark}
The setting of our attack for the CIKM paper is slightly different
from the setting discussed here: here the performance metric is $l(h)-l(h^{\star})$,
but in our attack, the metric is $\Pr(h(X)\neq h^{\star}(X))$. We
have $l(h)-l(h^{\star})\leq\Pr(h(X)\neq h^{\star}(X))$, so $\Pr(h(X)\neq h^{\star}(X))\leq\varepsilon$
implies an excess error $\varepsilon$, but the converse direction is
unclear.
\end{remark}
%
\begin{remark}
\cite{key-8} considers a noise setting where $\Pr(Y=1\mid X)=\phi(u^{\top}x)$
(this includes our attacking setting) for some function $\phi$. However,
theoretical results in \cite{key-8} are of a very general form, and
it is unclear what its label complexity bound is under our setting.
\end{remark}



%\begin{thebibliography}{1}
%\bibitem{key-1}Hanneke, Steve. \textquotedbl Theory of disagreement-based
%active learning.\textquotedbl{} Foundations and Trends® in Machine
%Learning 7.2-3 (2014): 131-309.
%
%\bibitem{key-2}Daniely, Amit. \textquotedbl Complexity theoretic
%limitations on learning halfspaces.\textquotedbl{} Proceedings of
%the forty-eighth annual ACM symposium on Theory of Computing. ACM,
%2016.
%
%\bibitem{key-4}Maria-Florina Balcan and Vitaly Feldman. Statistical
%active learning algorithms. In NIPS , pages 1295-- 1303, 2013.
%
%\bibitem{key-3}Klivans, Adam, and Pravesh Kothari. \textquotedbl Embedding
%Hard Learning Problems Into Gaussian Space.\textquotedbl{} Approximation,
%Randomization, and Combinatorial Optimization. Algorithms and Techniques
%(2014): 793.
%
%\bibitem{key-5}Yan, Songbai, and Chicheng Zhang. \textquotedbl Revisiting
%Perceptron: Efficient and Label-Optimal Learning of Halfspaces.\textquotedbl{}
%Advances in Neural Information Processing Systems. 2017.
%
%\bibitem{key-6}Pranjal Awasthi, Maria Florina Balcan, and Philip
%M Long . The power of localization for efficiently learning linear
%separators with noise. In Proceedings of the 46th Annual ACM Symposium
%on Theory of Computing , pages 449--458. ACM, 2014.
%
%\bibitem{key-7}M.-F. Balcan and P. M. Long. Active and passive learning
%o f linear separators under log-concave distribu- tions. In COLT ,
%2013.
%
%\bibitem{key-8}Agarwal, Alekh. \textquotedbl Selective sampling
%algorithms for cost-sensitive multiclass prediction.\textquotedbl{}
%International Conference on Machine Learning. 2013.
%\end{thebibliography}

==> Anon_Contents/continuous-case.tex <==
\subsection{Noisy Labels for the Continuous Case}
\label{subsec:continuous}

In the continuous, the model extraction problem becomes a regression
problem. In~\cite{HS14} the authors consider passive linear regression
with squared loss and provide an algorithm that achieves nearly
optimal convergence rate $\E [X^\top\hat{w}-Y]-\E[X^\top
  w^\star-Y]=\tilde{O} \left(\frac{C}{n}\right)$ where the constant
$C$ depends on the covariance matrix of $X$ and the error of the
optimal linear model $w^\star$. In~\cite{SM14} the authors point out
that unlike in the classification case, the $O(\frac{1}{n})$ cannot be
improved by active learning, but it provides an algorithm under a
stream-based querying model (in fact, they assume the algorithm can
draw $X$ from any distribution, which can be implemented by rejection
sampling with stream-based querying model) that achieves a learning
rate with a better constant factor $C$. Authors in~\cite{CKNS15}
consider active learning for maximum likelihood estimation (MLE) under the
assumption that the model is well-specified ($P(Y|X)$ is given by a
model in the model class) and that the Fisher information matrix does
not depend on label $y$ (this assumption holds for linear regression
and generalized linear models). It shows that a two-stage algorithm
achieves a nearly optimal convergence rate.

The main difficulties of computationally efficient active learning for
classification arise because of two factors: (1) how to efficiently
find a classifier with the minimum classification error rate; (2) how
to select examples for labeling. For (1), it has been shown that
optimizing the classification error rate (0-1 loss) with noise is hard
in general, and computational efficient solutions with theoretical
guarantees are only known under some assumptions of the hypothesis
space and noise conditions (for
example~\cite{chen2017near,key-3,key-5}). For (2), most existing
active learning algorithms maintain a candidate set of classifiers
either explicitly~\cite{H07} or
implicitly~\cite{chen2017near,DHM07,key-5}, and the noise tolerance is
achieved by repetitive querying as in Proposition~\ref{prop} or a
carefully designed sampling schedule to guarantee that the candidate
set is ``correctly shrunk'' with high
probability~\cite{DHM07,H07,key-5}. For regression, most loss
functions (for example the squared error, negative log likelihood) are
convex, and thus can be optimized efficiently. The labeling strategies
in regression are also different: instead of maintaining candidate
sets, active regression algorithms~\cite{SM14, CKNS15} often first
find a good sampling distribution that optimize some statistics of the
covariance matrix and then draw labeled samples from this
distribution. Such strategies tolerates noise naturally and de-noising
strategies like repetitive querying are not necessary.




==> Anon_Contents/macros.tex <==
\newcommand{\myparagraph}[1]{\vspace{0.1in}\noindent\textbf{#1}}
\newcommand{\myparnovspace}[1]{\vspace{0.0in}\noindent\textbf{#1}}
\newcommand{\myvspacenopar}{\vspace{0.1in}\noindent }
%\newcommand{\Sesy}{\S~}

\newtheorem{prop}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{lem}{Lemma}
\newtheorem*{notation*}{Notation}
\newtheorem*{rem*}{Remark}
\newtheorem{rem}{Remark}
\newcommand{\One}{\mathds{1}}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{experiment}{Experiment}

\theoremstyle{remark}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}

\newcommand{\ie}{\textit{i.e.}\@\xspace}
\newcommand{\eg}{\textit{e.g.}\@\xspace}
\newcommand{\etal}{\textit{et al.}\@\xspace}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\Y}{\ensuremath{\mathbf{Y}}}
\newcommand{\X}{\ensuremath{\mathbf{X}}}
\newcommand{\F}{\ensuremath{\mathcal{F}}}
\renewcommand{\L}{\ensuremath{\mathcal{L}}}
\renewcommand*{\O}{\ensuremath{\mathcal{O}}}
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\Ser}{\ensuremath{S}}
\newcommand{\Exp}{\ensuremath{\textup{\texttt{Exp}}}}
\newcommand{\uErr}{\ensuremath{\textup{Err}_u}}
\newcommand{\gErr}{\ensuremath{\textup{Err}_2}}
\newcommand{\Err}{\ensuremath{\textup{Err}}}
\newcommand{\sign}{\ensuremath{\textup{sign}}}
\newcommand{\negl}{\ensuremath{\textup{negl}}}
\newcommand{\tr}{\top}
\newcommand{\at}{\makeatletter @\makeatother}
\newcommand{\qquote}[1]{``#1''}


\newcommand{\Irene}[1]{\textcolor{blue}{[\textbf{Irene}: #1]}}
\newcommand{\Varun}[1]{\textcolor{green}{[\textbf{Varun}: #1]}}
\newcommand{\Somesh}[1]{\textcolor{purple}{[\textbf{Somesh}: #1]}}
\newcommand{\kc}[1]{\textcolor{orange}{[\textbf{Kamalika}: #1]}}
\newcommand{\Songbai}[1]{\textcolor{brown}{[\textbf{Songbai}: #1]}}
\newcommand{\todo}[1]{\textcolor{red}{[\textbf{ToDo}: #1]}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



==> Contents/eval.tex <==
\subsection{Non-Linear Models}
\label{subsec:nonlinear}

In this section, we report experimental results for extraction efficacy for non-linear models such as kernel SVMs and decision trees. Our experiments are designed to answer the following two questions: (1) Is QS active learning practically useful to extract non-linear models (\ie, kernel SVMs) in an oracle access setting?, and (2) Is active learning useful to extract non-linear models (\ie, decision trees) in scenarios where the ML server does not reveal any auxiliary information? As before, we use the same datasets as in Tram\`{e}r \etal~\cite{TZJRR16}. The continuous variables are made discrete by binning (\ie dividing into groups), and are then one-hot-encoded. Our experiments suggest that:

\begin{enumerate}
\itemsep0em
\item Utilizing the extended adaptive training (EAT) approach (refer \S~\ref{subsec:kSVM}) is efficient for extracting kernel SVMs. Our approach improves query complexity by 5$\times$-224$\times$.
\item Utilizing the IWAL algorithm (refer \S~\ref{subsec:iwal}) enables extracting a decision tree in the absence of {\em any} auxiliary information, with a nominal increase in query complexity (14$\times$). 
\end{enumerate}

\noindent{\bf Q1. Kernel SVM:} As discussed in \S~\ref{subsec:kSVM}, Tram\`{e}r \etal use {\em adaptive retraining} - a procedure to locate points close to the decision boundary - to obtain points used to seed their attack. Using these (labeled) points, they are able obtain the parameters which were used to instantiate the oracle using an extract-and-test approach (more specifically grid search). While techniques in active learning can not be used to expedite the grid search procedure, our experiments suggest that they are able to select more {\em informative} points \ie points of greater uncertainty, with far fewer queries. With insight from the work of Bordes \etal~\cite{LASVM}, we propose the {\em extended adaptive retraining approach} (refer \S~\ref{subsec:kSVM}) to obtain uncertain points. Additionally, we measure uncertainty with respect to a model that we train locally\footnote{such a local model is seeded with uniformly random points labeled by the oracle}, eliminating redundant queries to the oracle. To compare the efficiency of our algorithm, we re-execute the adaptive retraining procedure, and present our results in Table~\ref{table:kernelsvm}.

\begin{table}
\small
\centering
\begin{tabular}{c|c|c|c|c}
\hline
\toprule
\multicolumn{1}{c|}{\bf Dataset} & \multicolumn{2}{c|}{\bf Adaptive Retraining} & \multicolumn{2}{c}{\bf EAT}\\
\cline{2-5}
\multicolumn{1}{c|}{} &  Queries &  Accuracy &  Queries & Accuracy \\
\midrule
Mushroom   		& 11301	& 98.5	& 1001	& 94.5 \\
Breast Cancer  		& 1101	& 99.3	& 119	& 96.4 \\
Adult			& 10901	& 96.98	& 48	& 98.2 \\
Diabetes		& 901	& 98.5	& 166	& 94.8 \\
\bottomrule
\end{tabular}
	\compactcaption{\footnotesize \footnotesize Extraction of a kernel SVM model. Comparison of the query complexity and test accuracy (in $\%$) obtained running Tram\`{e}r \etal adaptive retraining vs. extended adaptive retraining.}
\label{table:kernelsvm}
\end{table}

It is clear that our approach is more query efficient in comparison to Tram\`{e}r \etal (between 5$\times$-224$\times$), with comparable test accuracy. These advantages stem from (a) using a more informative metric of uncertainty than the distance from the decision boundary, and (b) querying labels of only those points which the local model is uncertain about. 

\noindent{\bf Q2. Decision Trees:} Tram\`{e}r \etal propose a path finding algorithm to determine the structure of the server-hosted decision tree. They rely on the server's response to incomplete queries, and the addition of node identifiers to the generated outputs to recreate the tree. From our analysis presented in Table~\ref{aux}such flexibility is not readily available in most MLaaS providers. As discussed earlier (refer \S~\ref{subsec:iwal}), we utilize the IWAL algorithm proposed by Beygelzimer \etal~\cite{iwal:2010} that iteratively refines a learned hypothesis. It is important to note that the IWAL algorithm is more general, and does not rely on the information needed by the path finding algorithm. We present the results of extraction using the IWAL algorithm below in Table~\ref{table:iwal}.

\begin{table}
\small
\centering
\begin{tabular}{c|c|c|c|c}
\hline
\toprule
\multicolumn{1}{c|}{\bf Dataset} & \multicolumn{1}{|c|}{\bf Oracle} & \multicolumn{1}{c|}{\bf Path Finding} & \multicolumn{2}{c}{\bf IWAL}\\%& \multicolumn{2}{c|}{Langford Subsampled} \\%& \multicolumn{2}{c|}{Langford Mixed}\\
\cline{2-5}
	\multicolumn{1}{c|}{} & \multicolumn{1}{|c|}{ Accuracy} &  Queries &  Queries &  Accuracy\\% & num queries & Test Accuracy\\% & num queries & Test Accuracy\\
\midrule
Adult   	& 81.2	& 18323	& 244188& 80.2\\%	& 24426	& 69.1	& 48841	& 76.4\\
Steak  		& 52.1	& 5205	& 1334	& 73.1\\%	& 185	& 61.1	& 269	& 45.1\\
Iris		& 86.8	& 246	& 361	& 89.4\\%	& 35	& 84.1	& 85	& 84.1\\
GSShappiness	& 79	& 18907	& 254892& 79.3\\%	& 25621	& 69.1	& 51019	& 87.6\\
\bottomrule
\end{tabular}
\compactcaption{\footnotesize \footnotesize Extraction of a decision tree model. Comparison of the query complexity and test accuracy (in $\%$) obtained by running path finding (Tram\`{e}r \etal) vs. IWAL algorithm. The test accuracy  (in $\%$) of the server-hosted oracle is presented as a baseline.}
\label{table:iwal}
\vspace{-2mm}
\end{table}

In each iteration, the algorithm learns a new hypothesis, but the efficiency of the approach relies on the hypothesis used preceding the first iteration. To this end, we generate inputs uniformly at random. Note that in such a {\em uniform query generation} scenario, we rely on zero auxiliary information. We can see that while the number of queries required to launch such extraction attacks is greater than in the approach proposed by Tram\`{e}r \etal, such an approach obtains comparable test error to the oracle. While the authors rely on certain distributional assumptions to prove a label complexity result, we empirically observe success using the uniform strategy. Such an approach is truly powerful; it makes limited assumptions about the MLaaS provider and any prior knowledge.%The IWAL algorithm provides theoretical guarantees of convergence when (a) the labels are not noisy, and (b) the dataset used comes from the same distribution with which the oracle was trained. However, a practical attack may have noisy labels (\ie when attack dataset is labeled by a suboptimal oracle), or may not be from the same distribution (\ie sampled uniformly at random). However, we empirically observe success using the uniform strategy. Such an approach is truly powerful; it makes limited assumptions about the MLaaS provider and any prior knowledge.



